Grand Challenges around Designing Computers' Control Over Our Bodies

Advances in emerging technologies, such as on-body mechanical actuators and electrical muscle stimulation, have allowed computers to take control over our bodies. This presents opportunities as well as challenges, raising fundamental questions about agency and the role of our bodies when interacting with technology. To advance this research field as a whole, we brought together expert perspectives in a week-long seminar to articulate the grand challenges that should be tackled when it comes to the design of computers' control over our bodies. These grand challenges span technical, design, user, and ethical aspects. By articulating these grand challenges, we aim to begin initiating a research agenda that positions bodily control not only as a technical feature but as a central, experiential, and ethical concern for future human-computer interaction endeavors.

==> Sec-TechChallenges.tex <==
\section{Grand Challenges: Technology}

\subsection{Wearability}

Bodily control systems pose demanding challenges for ergonomic wearability. Actuators’ \textit{weight} is usually tied to how powerful they are; the considerable forces required for actuating the body result in systems of considerable weight, which can lead to fatigue when wearing. 
A second central property affecting ergonomic wearability is the device's \textit{rigidity}. It is well-known that technologies that are too rigid in their material reduce wearability [DON: REF [next steps]]. Yet, we note some correlation between an actuator's strength and rigidity: not only are most actuators rigid (see mechanical exoskeletons), but the more forceful they are, the more rigid they need to be. Rigid and oftentimes rather bulky actuators stand in contrast to the “softness” of the human body, leading to reduced \textit{body conformity} and possibly even interfering with the user's motor activities. In addition, more forceful actuators tend to produce more heat, which can further reduce \textit{thermal comfort}. As such, we highlight the need for technical advances in soft(er) body actuating technologies that are more lightweight and conformable to the body, while being able to exert the forces required for actuating the body.  
Developers of wearable systems designed to control our bodies should also consider how users can mount and dismount them on the body~\cite{knibbe_skillsleeves}. A technical challenge is to design systems such that the user can mount and dismount it without the help of another person. 


\subsection{Personalization}

Bodily control systems present strong demands on personalization for individual users, both in their hardware and software components. 
All the systems we present in this article are either bespoke research systems or designed in small numbers, hence associated with significant development time and cost. In specific applications, such as body-controlling prosthetics, the high cost of developing a solution specifically for an individual can be acceptable. However, this would prevent more widespread application in broader areas. Scaling up to mass fabrication can considerably reduce cost, since the more identical devices are produced, the cheaper each one typically becomes. However, a “one-size-fits-all” approach stands in stark contrast to the fact that each body is different. It remains an open challenge how to effectively support personalization of bodily control systems for individual users while drawing from the benefits of mass-manufacturing processes in a cost-efficient way. A promising direction is to offer physical customization options within mass-manufactured devices, such as modular reconfiguration or adjustable mounts. Another direction involves digital design tools alongside digital fabrication processes, which allow for computationally tailoring a device design for an individual user, for instance by capturing the user's body dimensions or individual range of motion \cite{WRLKit}.
Once deployed on the body, the system's interactive behavior needs to be further calibrated for individual differences such as body weight, height, skin thickness etc.  Calibrating a body control system is even harder as it may need to sense specific physiological signals and actuate specific muscles or body parts~\cite{knibbe_automaticEMS_2017,Gange_Knibbe_2021}. This may require a combination of approaches; firstly, accurate sensor/actuator placement and calibration for individual factors is important to successfully achieve the goals of bodily control systems. Due to the complexity of the human body, this calibration often takes time and both physical and mental effort, which may reduce the user experience of the body control device. This is further aggravated, as systems may need to be recalibrated during use due to changes in body state or environmental factors. Identifying the optimal time as to when and how the system needs to be recalibrated is essential. Hence, designing for minimal calibration is a highly important, yet challenging task~\cite{Gange_Knibbe_2021}. Promising directions here include: leveraging black-box optimisation techniques~\cite{Gange_Knibbe_2021}; building on user's informed decisions to ease semi-automatic interactive calibration~\cite{Pohl2018EMSCalibration}; and using closed-loop feedback from the same modality (e.g., EMS stimulation-EMG measurement)~\cite{knibbe_automaticEMS_2017}.


\subsection{Ease of Prototyping}

Today, developing bodily control systems remains a costly and time-consuming endeavor, exclusively restricted to a small group who have the specific expertise. This prevents a larger group of stakeholders from exploring, ideating, designing, and ultimately deploying solutions. It remains a grand challenge to develop accessible solutions that will allow a broad community of non-roboticists, such as interaction designers, makers or application domain experts, to prototype their interactive solutions, and do so in a cost-efficient, easy and rapid way. 


\subsection{Maximizing Capability}

Knowing a system’s technical capacity to control a human body is paramount to the scope of possible applications. We must develop a formal structure to report the technical capacity if we apply such systems for any relevant use case. For instance, if we are to move uphill, we must know the upper limit capacity of the system. Moreover, for systems initiating or taking over motor abilities, for instance, through EMS technology, the system’s maximum performance must be known to elicit the required effort and not more or less. There are no formal standards or frameworks for such technical reports, which is a grand challenge for such systems’ development and future applications. 


==> Tables/118-challenges-table.tex <==
% % Required packages for this table:
% % \usepackage{xltabular}  % Combines longtable + tabularx for auto-width adjustment
% % \usepackage[table]{xcolor}
% %
% % Or alternatively:
% % \usepackage{xltabular}
% % \usepackage{colortbl}
% % \usepackage{xcolor}
% %
% % Note: Borders are automatically included in this table using \hline and vertical rules
% %
% % Note: Using xltabular with X columns for automatic width adjustment
% % Columns automatically expand to fit the full page width (\textwidth)
% % Proportional widths: Entry (2.0X), Final Label (1.3X), Design (1.2X),
% % Our Interpretation (0.7X), Method/Technology/User/Society (0.7X each)
% % Sum = 8.0X (matches 8 columns) - automatically adjusts to any page width
% \begin{xltabular}{\textwidth}{|>{\hsize=2.0\hsize}X|>{\hsize=1.3\hsize}X|>{\hsize=0.7\hsize}X|>{\hsize=0.7\hsize}X|>{\hsize=0.7\hsize}X|>{\hsize=0.7\hsize}X|>{\hsize=0.7\hsize}X|>{\hsize=1.2\hsize}X|}
%     \caption{The table lists all entries gathered from discussions and groups them across themes such as method, technology, user, society, and design.}
%     \label{tab:list-of-total-grand-challenges}\\
%     \hline
%     %\rowcolor[HTML]{4DD0E1}
%     \textbf{Entry} &
%       \textbf{Final Label} &
%       \textbf{Our Interpretation} &
%       \textbf{Method} &
%       \textbf{Technology} &
%       \textbf{User} &
%       \textbf{Society} &
%       \textbf{Design} \\
%     \hline
%     \endfirsthead
%     %
%     \hline
%     \textbf{Entry} &
%       \textbf{Final Label} &
%       \textbf{Our Interpretation} &
%       \textbf{Method} &
%       \textbf{Technology} &
%       \textbf{User} &
%       \textbf{Society} &
%       \textbf{Design} \\
%     \hline
%     \endhead
%     %
%     \hline
%     \endfoot
%     \hline
%     \endlastfoot
%     \rowcolor[HTML]{FFFFFF}
%     Parasite, friend, part of me &
%       Parasite vs Assistant &
%        &
%        &
%        &
%        &
%        &
%       Parasite vs Assistant \\
%     \rowcolor[HTML]{E0F7FA}
%     How should it be designed to allow integration (rather than a parasite an assistant into your body/mind) &
%       Parasite vs Assistant &
%        &
%        &
%        &
%        &
%        &
%       Parasite vs Assistant \\
%     \rowcolor[HTML]{FFFFFF}
%     Laziness &
%       Laziness &
%        &
%        &
%        &
%       Laziness &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Spaces of control &
%       Spaces of control &
%        &
%        &
%        &
%        &
%       Spaces of control &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Computer-initiated vs Human/Body Initiated &
%       Initiative &
%        &
%        &
%        &
%        &
%        &
%       Initiative \\
%     \rowcolor[HTML]{E0F7FA}
%     Implicit control \textless{}=\textgreater Explicit control &
%       Implicit vs Explicit &
%        &
%        &
%        &
%        &
%        &
%       Implicit vs Explicit \\
%     \rowcolor[HTML]{FFFFFF}
%     Beliefs about capability/competence &
%       Belief of competence &
%        &
%        &
%        &
%       Belief of competence &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Sense of agency vs Feeling of agency &
%       Agency &
%        &
%        &
%        &
%        &
%        &
%       Agency \\
%     \rowcolor[HTML]{FFFFFF}
%     Inattentional/attentional action binding &
%       Measurement of sense of agency &
%        &
%       Measurement of sense of agency &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Body as Canvas + Social environment cultural values &
%       Social environment and cultural values \newline Body as canvas &
%        &
%        &
%        &
%        &
%       Social environment and cultural values &
%       Body as canvas \\
%     \rowcolor[HTML]{FFFFFF}
%     Safety, feeling safe and comfortable. No unpleasant surprises &
%       Feeling of safety. Comfort. \newline Communicating system's intentions &
%        &
%        &
%        &
%       Feeling of safety. Comfort. &
%        &
%       Communicating system's intentions \\
%     \rowcolor[HTML]{E0F7FA}
%     Control \textless{}=\textgreater Agency &
%       Control vs. Agency &
%        &
%        &
%        &
%        &
%        &
%       Control vs. Agency \\
%     \rowcolor[HTML]{FFFFFF}
%     Control-change tradeoff (is not zero-sum) &
%       Transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Transparency/Informed transfer of control &
%       Informed transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Informed transfer of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Surrendering/ giving up/losing control &
%       Transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Relation with augmented technology using Play Theory (4 play types) &
%       Play Theory &
%        &
%        &
%        &
%        &
%        &
%       Play Theory \\
%     \rowcolor[HTML]{FFFFFF}
%     Persuasion &
%       Transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Regain control &
%       Transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Level of personalization and individual preferences &
%       Personalization and Customization &
%        &
%        &
%        &
%       Personalization and Customization &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Level of automation and sense of agency &
%       Automation vs Agency &
%        &
%        &
%        &
%        &
%        &
%       Automation vs Agency \\
%     \rowcolor[HTML]{FFFFFF}
%     Signals, entrypoints, targets &
%       Design space &
%        &
%        &
%        &
%        &
%        &
%       Design space \\
%     \rowcolor[HTML]{E0F7FA}
%     Signal intensity vs User disposition to obey &
%       Control signal intensity \newline User obedience &
%        &
%        &
%       Control signal intensity &
%       User obedience &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Lack of knowledge on responses of our body's physiology to external stimulations &
%       Elicitated responses &
%        &
%        &
%       Elicitated responses &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Ethical challenges &
%       Ethics &
%        &
%        &
%        &
%        &
%       Ethics &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Who is in control? &
%       Ownership of control &
%        &
%        &
%        &
%        &
%        &
%       Ownership of control \\
%     \rowcolor[HTML]{E0F7FA}
%     adaptation versus adoption between humans and computers – and their experiential implications &
%       Adaptation vs Adoption &
%        &
%        &
%        &
%        &
%        &
%       Adaptation vs Adoption \\
%     \rowcolor[HTML]{FFFFFF}
%     Computer-Supported Control over Body (CSCB) &
%       CSCB &
%        &
%        &
%        &
%        &
%        &
%       CSCB \\
%     \rowcolor[HTML]{E0F7FA}
%     Explainable and transparent intervention approaches &
%       Explainability and Transparency &
%        &
%        &
%        &
%        &
%        &
%       Explainability and Transparency \\
%     \rowcolor[HTML]{FFFFFF}
%     What is our sun? Try to identify the extent of symbiosis/integration/manipulation. &
%       Limits of control &
%        &
%        &
%        &
%        &
%        &
%       Limits of control \\
%     \rowcolor[HTML]{E0F7FA}
%     What scenarios or applications should we build for? &
%       Applications &
%        &
%        &
%        &
%        &
%        &
%       Applications \\
%     \rowcolor[HTML]{FFFFFF}
%     How does the computer understand what it can control? &
%       Control representation &
%        &
%        &
%       Control representation &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     \begin{tabular}[c]{@{}l@{}}Redirection is fun.\\ But its really interesting in multi-user systems.\\ What I am doing and what you see can be entirely different.\\ How do I control this?\\ What does this control mean for trust?\end{tabular} &
%       Trust &
%        &
%        &
%        &
%       Trust &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Can we benchmark control? &
%       Benchmark &
%        &
%       Benchmark &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Do we understand Control well enough to think about Control in Augmentation Systems? &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Definition of Control &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Defining control, shared control, augmentation, intervention &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Co-control &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Impact of loss of control (e.g., facial paralysis leads to loss of control, cannot talk/chew/emote as desired). &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{FFFFFF}
%     How does loss of sense of body impact what control means (e.g., prosthetics). &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{E0F7FA}
%     What do we mean when we say the computer has "control" over one's body? &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{FFFFFF}
%     What do we mean by the body? &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Location (space) &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Location (body) &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{E0F7FA}
%     What is the non-invasive EMG \textless{}\textgreater EMS equivalent for ?? \textless{}\textgreater GVS &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Is the goal to train the body or is the tech always going to be needed. &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Computer Supported Control over Body &
%       Concept of control &
%        &
%        &
%        &
%        &
%        &
%       Concept of control \\
%     \rowcolor[HTML]{FFFFFF}
%     What are the most pressing real world applications &
%       Applications &
%        &
%        &
%        &
%        &
%        &
%       Applications \\
%     \rowcolor[HTML]{E0F7FA}
%     Voluntarily giving up control $\sim$social contract theory &
%       Transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Zero-sum game? Giving up control and taking back maybe give up one thing and get back something else &
%       Transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Freedom &
%       Transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Power relationships (social) &
%       came from conversation on what does control mean in a social setting Transfer of control &
%       came from conversation on what does control mean in a social setting &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{E0F7FA}
%     Culture - that "computer/machine" is coming close to my body - how do I like that? I would not let anyone touch my shadow! &
%       Transfer of control &
%        &
%        &
%        &
%        &
%        &
%       Transfer of control \\
%     \rowcolor[HTML]{FFFFFF}
%     Intentionality vs relationality &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Scale vs hierarchy &
%       Came out of conversation about telling a 3d printer what to print and the printer performing that task with no volition \newline Trade-offs &
%       Came out of conversation about telling a 3d printer what to print and the printer performing that task with no volition &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{FFFFFF}
%     Macro vs micro goals &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Interface vs control &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{FFFFFF}
%     Body vs mind &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Does control over the human body mean to control body and mind? &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{FFFFFF}
%     Augmentation vs control &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Sense of agency vs feeling of agency &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{FFFFFF}
%     Long-term control device vs in-lab/short term &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Wearable vs environmental &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{FFFFFF}
%     Dystopian vs utopian &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Choice vs not - who is deciding &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{FFFFFF}
%     Trade-off between agency and automation &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Assist/augment/replace &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{FFFFFF}
%     Do we mean to help, to augment or to replace human behavior? &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Transcendent responsibility &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{FFFFFF}
%     Calibration &
%       came from conversation about GVS needing to be personalized \newline Technology &
%       came from conversation about GVS needing to be personalized &
%        &
%       Technology &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Reading and writing GVS signals &
%       Technology &
%        &
%        &
%       Technology &
%        &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Quantify impact of aging on the senses &
%       Adoption &
%        &
%        &
%        &
%       Adoption &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Interaction &
%       Interaction &
%        &
%        &
%        &
%       Interaction &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     (Inter)action outcome &
%       Interaction &
%        &
%        &
%        &
%       Interaction &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Temporal scale of control &
%       Interaction &
%        &
%        &
%        &
%       Interaction &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Implications for long-term use &
%       Adoption &
%        &
%        &
%        &
%       Adoption &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Time (duration, frequency) &
%       Interaction &
%        &
%        &
%        &
%       Interaction &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Methods for understanding control &
%       Understanding control \newline Backing Theory &
%        &
%       Understanding control &
%        &
%        &
%        &
%       Backing Theory \\
%     \rowcolor[HTML]{E0F7FA}
%     SDT \textless{}\textgreater control &
%       self determination theory \newline Backing Theory &
%       self determination theory &
%        &
%        &
%        &
%        &
%       Backing Theory \\
%     \rowcolor[HTML]{FFFFFF}
%     Placebo - visual augmentations to face/body &
%       came out of conversation about adding bunny ears to face and if that can lead to an identity over time and if that identity has an impact on behavior \textgreater proteus effect or on self-perception \textgreater placebo effect (e.g., looking younger facial filter) \newline User-centric &
%       came out of conversation about adding bunny ears to face and if that can lead to an identity over time and if that identity has an impact on behavior \textgreater proteus effect or on self-perception \textgreater placebo effect (e.g., looking younger facial filter) &
%        &
%        &
%       User-centric &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Proteus effect &
%       User-centric &
%        &
%        &
%        &
%       User-centric &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Effect on perception of self &
%       User-centric &
%        &
%        &
%        &
%       User-centric &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Level of personalization &
%       User-centric &
%        &
%        &
%        &
%       User-centric &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Personalized continuum &
%       User-centric &
%        &
%        &
%        &
%       User-centric &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Perception &
%       User-centric &
%        &
%        &
%        &
%       User-centric &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Experience &
%       User-centric &
%        &
%        &
%        &
%       User-centric &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Explainable intervention &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{FFFFFF}
%     Intentionality transparency &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{E0F7FA}
%     (How) do we make control transparent to the user? &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{FFFFFF}
%     Lack of knowledge of mechanism &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{E0F7FA}
%     Visibility &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{FFFFFF}
%     Awareness &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{E0F7FA}
%     Action &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{FFFFFF}
%     Anticipation &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{E0F7FA}
%     Getting users to trust systems to try &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{FFFFFF}
%     Familiarity/getting used to sensation &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{E0F7FA}
%     Can the human object to the control? &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{FFFFFF}
%     Do we plan to give control back to the human ? &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{E0F7FA}
%     Existential fusion &
%       Communicating and Signalling Control &
%        &
%        &
%        &
%        &
%        &
%       Communicating and Signalling Control \\
%     \rowcolor[HTML]{FFFFFF}
%     Body norms/accessibility/impairment/different bodies &
%       Accessibility &
%        &
%        &
%        &
%        &
%        &
%       Accessibility \\
%     \rowcolor[HTML]{E0F7FA}
%     Accessibility - who do we design for? Age? &
%       Accessibility &
%        &
%        &
%        &
%        &
%        &
%       Accessibility \\
%     \rowcolor[HTML]{FFFFFF}
%     Devices (progressively adaptive as the inner ear changes with age, exposure). &
%       Accessibility &
%        &
%        &
%        &
%        &
%        &
%       Accessibility \\
%     \rowcolor[HTML]{E0F7FA}
%     Level of support/control needed for novice vs. professional &
%       Accessibility &
%        &
%        &
%        &
%        &
%        &
%       Accessibility \\
%     \rowcolor[HTML]{FFFFFF}
%     Body manipulations (physically, can it take other forms?) &
%       Modalities &
%        &
%       Modalities &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Black mirror scenarios &
%       Imaginary scenario &
%        &
%       Imaginary scenario &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Implicit vs Explicit / psych vs physical &
%       Trade-offs &
%        &
%        &
%        &
%        &
%        &
%       Trade-offs \\
%     \rowcolor[HTML]{E0F7FA}
%     Manipulation &
%       Manipulation &
%        &
%        &
%        &
%        &
%        &
%       Manipulation \\
%     \rowcolor[HTML]{FFFFFF}
%     Understanding of the body's relations to external structures &
%       Bodily understanding &
%        &
%        &
%        &
%        &
%        &
%       Bodily understanding \\
%     \rowcolor[HTML]{E0F7FA}
%     Granularity of control &
%       Granularity &
%        &
%        &
%        &
%        &
%        &
%       Granularity \\
%     \rowcolor[HTML]{FFFFFF}
%     How many wearables do we expect &
%       adoption of wearables &
%        &
%        &
%        &
%       adoption of wearables &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Whole body vs components &
%       Body parts &
%        &
%        &
%        &
%       Body parts &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Cultivate value ( feet) &
%       Cultivate value &
%        &
%        &
%        &
%        &
%       Cultivate value &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Intentionality &
%        &
%        &
%        &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Are we having a reductionalist approach? &
%        &
%        &
%        &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Who gets to design the system? Who has a say? I.e., who controls the design process or the computer? &
%        &
%        &
%        &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     How do we design the system to achieve the level of control? &
%        &
%        &
%        &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Do we want to create dependency or create ability to be then learn to be in control? &
%        &
%        &
%        &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{FFFFFF}
%     Human changes at different timescales (not just long ones) and not always in the same directions (e.g., not always getting either better or worse), affective states induce temporary changes's in capabilities) &
%        &
%        &
%        &
%        &
%        &
%        &
%        \\
%     \rowcolor[HTML]{E0F7FA}
%     Affective states alter perception and acceptability etc. &
%        &
%        &
%        &
%        &
%        &
%        &
%        \\
%     \end{xltabular}

==> Tables/GrandChallengesTable.tex <==
% \begin{table*}
% \caption{Summary of Grand Challenges}
% \label{tbl:GrandChallenges}
% \centering
% \begin{tabular}{ l >{\hangindent=18pt} p{0.85\linewidth} }
% \toprule
% Grouping& Challenge \\
% \midrule
% Technology & \textbf{Wearability:} Challenges related to ergonomic wearability of bodily control systems, including weight, rigidity, body conformity, and thermal comfort. \\
% & \textbf{Personalization:} Strong demands on personalization of hardware and software components for individual users while considering mass-manufacturing processes. \\
% & \textbf{Ease of Prototyping:} Developing accessible solutions for non-experts to prototype bodily control systems in a cost-efficient and rapid way. \\
% & \textbf{Maximizing Capability:} Need for formal standards to report the technical capacity of bodily control systems for various applications. \\ \addlinespace
% Design & \textbf{Designing for Shared Agency:} Balancing control between user and technology to ensure shared agency and user empowerment. \\
% & \textbf{Seamless Transitions between Human Autonomy and System Control:} Ensuring smooth transitions between user autonomy and system control to maintain user trust and comfort. \\
% & \textbf{Aesthetics:} Designing aesthetically pleasing systems that are acceptable across changing states and user preferences. \\ \addlinespace
% Ethics & \textbf{Safety:} Addressing safety issues arising from direct control over human physiology, including unintended reflexive actions and environmental risks. \\
% & \textbf{Accountability:} Clarifying accountability when systems malfunction or cause harm due to shared control over the human body. \\
% & \textbf{Health:} Mitigating potential physical and mental health risks from long-term use, such as injury, cognitive overload, and dependency. \\
% & \textbf{Inclusivity:} Ensuring inclusive design that accounts for diverse bodily characteristics and avoids reinforcing disparities. \\
% & \textbf{Cultural Sensitivity:} Considering cultural sensitivities and practices related to body autonomy, privacy, and control in design and deployment. \\
% & \textbf{Perception of Self, Objection and Exit:} Ensuring users can object to or exit from systems that control their bodies, avoiding coercion and addressing power dynamics. \\ \addlinespace
% Users & \textbf{Evaluation Framework:} Understanding when, why, and how to evaluate user experiences, ensuring studies capture both short-term and long-term impacts. \\
% & \textbf{Shared Experiences:} Facilitating shared experiences with bodily control systems while managing safety, accessibility, and engagement. \\
% & \textbf{Measuring Bodily Control Systems:} Developing reliable measures for agency, user experience, and interaction qualities in bodily control systems. \\
% \bottomrule
% \end{tabular}
% \end{table*}


\begin{table*}[t]
\centering
\caption{Summary of Grand Challenges}
\begin{tabular}{p{1.4cm}p{13cm}}
\toprule
\textbf{Grouping} & \textbf{Challenge} \\
\midrule
\multirow{4}{*}{Technology} 
& \textbf{Wearability}: Challenges related to ergonomic wearability of bodily control systems, including weight, rigidity, body conformity, and thermal comfort. \\
& \textbf{Personalization}: Strong demands on personalization of hardware and software components for individual users while considering mass-manufacturing processes. \\
& \textbf{Ease of Prototyping}: Developing accessible solutions for non-experts to prototype bodily control systems in a cost-efficient and rapid way. \\
& \textbf{Maximizing Capability}: Need for formal standards to report the technical capacity of bodily control systems for various applications. \\
\midrule
\multirow{3}{*}{Design} 
& \textbf{Designing for Shared Agency}: Balancing control between user and technology to ensure shared agency and user empowerment. \\
& \textbf{Seamless Transitions between Human Autonomy and System Control}: Ensuring smooth transitions between user autonomy and system control to maintain user trust and comfort. \\
& \textbf{Aesthetics}: Designing aesthetically pleasing systems that are acceptable across changing states and user preferences. \\
\midrule
\multirow{6}{*}{Ethics} 
& \textbf{Safety}: Addressing safety issues arising from direct control over human physiology, including unintended reflexive actions and environmental risks. \\
& \textbf{Accountability}: Clarifying accountability when systems malfunction or cause harm due to shared control over the human body. \\
& \textbf{Health}: Mitigating potential physical and mental health risks from long-term use, such as injury, cognitive overload, and dependency. \\
& \textbf{Inclusivity}: Ensuring inclusive design that accounts for diverse bodily characteristics and avoids reinforcing disparities. \\
& \textbf{Cultural Sensitivity}: Considering cultural sensitivities and practices related to body autonomy, privacy, and control in design and deployment. \\
& \textbf{Perception of Self, Objection and Exit}: Ensuring users can object to or exit from systems that control their bodies, avoiding coercion and addressing power dynamics. \\
\midrule
\multirow{3}{*}{Users} 
& \textbf{Evaluation Framework}: Understanding when, why, and how to evaluate user experiences, ensuring studies capture both short-term and long-term impacts. \\
& \textbf{Shared Experiences}: Facilitating shared experiences with bodily control systems while managing safety, accessibility, and engagement. \\
& \textbf{Measuring Bodily Control Systems}: Developing reliable measures for agency, user experience, and interaction qualities in bodily control systems. \\
\bottomrule
\end{tabular}
\label{tbl:GrandChallenges}
\end{table*}
